Youtu-Parsing-Omni: One Encoder, One Schema, All Modalities

We present Youtu-Parsing-Omni, an omni-modal parser that converts documents, images, audio, and video into structured records grounded in space and time, providing a perception layer for agents that read, locate, and cite evidence across modalities. Its design rests on one encoder for every modality and one schema for every task. Youtu-Omni-Encoder, initialized from a pre-trained language model to strengthen text reading, encodes all modalities with shared weights in a unified space-time coordinate system, and a few fusion layers let video frames attend to concurrent audio, bringing cross-modal fusion and temporal alignment into perception itself. OmniSchema unifies the outputs of all ten parsing tasks, allowing a single self-evolving post-training procedure, OmniSchema-Aware On-Policy Distillation (OSAD), to provide a shared token-role-based objective across tasks. In each round, the model is trained on its own rollouts against token-level targets from a reference-conditioned copy of itself, which is then refreshed with the trained weights, so that the parser and its supervision co-evolve. With a single 5 B-parameter checkpoint, Youtu-Parsing-Omni achieves state-of-the-art performance on OmniDocBench v1.6 (96.96 Overall) and leads all open-weight models on OmniParsingBench (75.08 Avg.), with its advantage concentrated on audio and video. It also achieves the best overall chart-parsing score (95.02) and the highest exact chemical-fingerprint agreement among compared systems, and matches a dedicated optical-music model in character-level transcription of typeset sheet music while staying far ahead of general-purpose systems. Code and model weights are publicly available.

==> tables/automatic_speech_recognition_chinese.tex <==
\begin{table*}[!t]
\centering
\caption{\textbf{Chinese ASR} (CER, \%, lower is better). Baseline numbers are taken from the comparison compiled by VITA-Audio~\cite{VITA-Audio} (its Tab.~4 and appendix), which takes them in part from the original reports.}
\label{tab:asr-chinese}
\begin{adjustbox}{max width=0.60\textwidth}
\begin{tabular}{c l c}
\toprule
{Datasets} & {Model} & CER (\%) $\downarrow$ \\


\midrule
\multirow{11}{*}{\begin{tabular}[c]{@{}c@{}}{AISHELL-1}~\hfilll~\cite{AISHELL_1} \end{tabular}} 
& Qwen2-Audio-base~\hfilll~\cite{Qwen2-Audio} & 1.52 \\ 
& Baichuan-Audio-base~\hfilll~\cite{Baichuan-Audio} & 1.93 \\
& Freeze-Omni~\hfilll~\cite{Freeze-Omni} & 2.48 \\
& LUCY~\hfilll~\cite{LUCY} & 2.40 \\
& Step-Audio-chat~\hfilll~\cite{Step-Audio} & 2.14 \\
& Qwen2.5-Omni~\hfilll~\cite{Qwen2.5-Omni} & \textbf{1.13} \\
& VITA-Audio~\hfilll~\cite{VITA-Audio} & 1.94 \\

\cmidrule{2-3}

& \cellcolor{youtuBlue!7}\oursmark\OurMethodBF & \cellcolor{youtuBlue!7}2.40 \\


\midrule
\multirow{11}{*}{\begin{tabular}[c]{@{}c@{}}{WenetSpeech}~\hfilll~\cite{WenetSpeech} \\ \textit{test-meeting} | \textit{test-net} \end{tabular}}
& Qwen2-Audio-base~\hfilll~\cite{Qwen2-Audio} & 8.40 | 7.64 \\ 
& Baichuan-Audio-base~\hfilll~\cite{Baichuan-Audio} & 13.28 | 10.13 \\
& Freeze-Omni~\hfilll~\cite{Freeze-Omni} & 13.46 | 11.80 \\
& VITA-1.5~\hfilll~\cite{VITA-1.5} & 10.00 | 8.40 \\
& LUCY~\hfilll~\cite{LUCY} & 10.42 | 8.78 \\
& Step-Audio-chat~\hfilll~\cite{Step-Audio} & 10.83 | 9.47 \\
& Qwen2.5-Omni~\hfilll~\cite{Qwen2.5-Omni} & 7.71 | \textbf{6.04} \\
& VITA-Audio~\hfilll~\cite{VITA-Audio} & \textbf{7.12} | 6.90 \\

\cmidrule{2-3}

& \cellcolor{youtuBlue!7}\oursmark\OurMethodBF & \cellcolor{youtuBlue!7}11.44 | 8.19 \\



\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}


==> tables/automatic_speech_recognition_english.tex <==


\begin{table*}[!t]
\centering
\caption{\textbf{English ASR} (WER, \%, lower is better). Baseline numbers are taken from the comparison compiled by VITA-Audio~\cite{VITA-Audio} (its Tab.~4 and appendix), which takes them in part from the original reports.}
\label{tab:asr-english}
\begin{adjustbox}{max width=0.60\textwidth}
\begin{tabular}{c l c}
\toprule
{Datasets} & {Model} & WER (\%) $\downarrow$ \\


\midrule
\multirow{11}{*}{\begin{tabular}[c]{@{}c@{}}{LibriSpeech}~\hfilll~\cite{Librispeech} \\ \textit{test-clean} | \textit{test-other}\end{tabular}} 
& Qwen2-Audio-base~\hfilll~\cite{Qwen2-Audio} & \textbf{1.74} | \textbf{4.04} \\ 
& Baichuan-Audio-base~\hfilll~\cite{Baichuan-Audio} & 3.02 | 6.04 \\
& Freeze-Omni~\hfilll~\cite{Freeze-Omni} & 3.82 | 9.79 \\
& VITA-1.5~\hfilll~\cite{VITA-1.5} & 3.40 | 7.50 \\
& LUCY~\hfilll~\cite{LUCY} & 3.36 | 8.05 \\
& Step-Audio-chat~\hfilll~\cite{Step-Audio} & 3.19 | 10.67 \\
& Qwen2.5-Omni~\hfilll~\cite{Qwen2.5-Omni} & 2.37 | 4.21 \\
& VITA-Audio~\hfilll~\cite{VITA-Audio} & 2.00 | 4.60 \\

\cmidrule{2-3}

& \cellcolor{youtuBlue!7}\oursmark\OurMethodBF & \cellcolor{youtuBlue!7}2.33 | 6.12 \\


\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}


==> tables/efficiency.tex <==
\begin{table}[!t]
\centering
\caption{\textbf{Inference cost on documents.} All models run on the same hardware, \tbd[accelerator], with \tbd[inference engine] over the \tbd{} pages of OmniDocBench v1.6. Throughput is measured at batch size \tbd; latency is per page at batch size $1$.}
\label{tab:efficiency}
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l r c ccc}
\toprule
\tabhead Model & Params & OmniDocBench & Pages/s$\uparrow$ & Latency (s)$\downarrow$ & Peak memory (GB)$\downarrow$ \\
\midrule
\OurMethodV1~\hfilll~\cite{Youtu-Parsing}       & $2.5$\,B & 93.74 & \tbd & \tbd & \tbd \\
MinerU2.5-Pro~\hfilll~\cite{MinerU2.5-Pro}       & $1.2$\,B & 95.75 & \tbd & \tbd & \tbd \\
PaddleOCR-VL-1.6~\hfilll~\cite{PaddleOCR-VL-1.6} & $0.9$\,B & 96.34 & \tbd & \tbd & \tbd \\
\midrule
\rowcolor{youtuBlue!7}\oursmark\OurMethodBF   & $5$\,B & 96.96 & \tbd & \tbd & \tbd \\
\bottomrule
\end{tabular}
\end{table}


==> tables/fusion_sweep.tex <==
\begin{table}[!t]
\centering
\caption{\textbf{In-encoder fusion is a function of clip length: it helps on medium and long videos and not on short ones.} Video-MME by clip length (higher is better) after $1{,}000$ long-context fine-tuning steps per variant, in the proxy setting of Subsec.~\ref{subsec:eval-analysis} and without parsing data. Best value in each column in \textbf{bold}. \emph{None} disables cross-modal attention; the remaining variants fuse in all layers, in the middle layers, or in the late layers, at the fusion probability $p_{\mathrm{fus}}$ of Subsec.~\ref{subsec:omni-video}. The final model combines the middle and late placements. Within this sweep the overall spread ($66.7$--$68.6$) is smaller than the differences between clip lengths, which is why the columns rather than the overall score carry the conclusion.}
\label{tab:fusion}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l ccc c}
\toprule
\tabhead Fusion variant (proxy) & Short & Medium & Long & Overall \\
\midrule
none                              & \best{78.6} & 67.8          & 57.8          & 68.0 \\
all layers                        & 76.1        & 67.9          & 56.1          & 66.7 \\
all layers, $p_{\mathrm{fus}}=0.8$     & 77.2        & 69.2          & 57.3          & 67.9 \\
middle layers, $p_{\mathrm{fus}}=0.8$  & 77.7        & 68.9          & 58.0          & 68.2 \\
late layers, $p_{\mathrm{fus}}=0.8$    & 77.8        & \best{69.3}   & \best{58.7}   & \best{68.6} \\
\bottomrule
\end{tabular}
\end{table}


==> tables/gen_omnidocbench_full.tex <==
\begin{table}[!t]
\centering
\caption{\textbf{OmniDocBench v1.6: \OurMethod ranks first among all systems and is on par with TeleOCR ($0.05$ apart).} Full set, official evaluation code. Overall $=\big((1-\text{Text Edit})\cdot100+\text{Formula CDM}+\text{Table TEDS}\big)/3$; Edit metrics are lower-is-better. \textbf{Bold} and \underline{underline}: best and second best in each column.
}
\label{tab:omnidocbench-full}
\small\setlength{\tabcolsep}{4.5pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l l r cccccc}
\toprule
\tabhead Model & Type & Params & Overall$\uparrow$ & Text Edit$\downarrow$ & Formula CDM$\uparrow$ & TEDS$\uparrow$ & TEDS-S$\uparrow$ & Read.\ Order Edit$\downarrow$ \\
\midrule
TeleOCR~\hfilll~\cite{TeleOCR} & specialized & $1.2$\,B & \second{96.91} & \second{0.0267} & 96.59 & \best{96.82} & \second{98.18} & 0.1184 \\
OvisOCR2~\hfilll~\cite{OvisOCR2} & specialized & $0.8$\,B & 96.47 & \best{0.0265} & \second{97.49} & 94.58 & 96.98 & \second{0.1120} \\
PaddleOCR-VL-1.6~\hfilll~\cite{PaddleOCR-VL-1.6} & specialized & $0.9$\,B & 96.34 & 0.0326 & \best{97.53} & 94.76 & 97.10 & 0.1278 \\
MinerU2.5-Pro~\hfilll~\cite{MinerU2.5-Pro} & specialized & $1.2$\,B & 95.75 & 0.0360 & 97.45 & 93.42 & 95.92 & 0.1200 \\
GLM-OCR~\hfilll~\cite{GLM-OCR} & specialized & $0.9$\,B & 95.22 & 0.0440 & 97.18 & 92.83 & 95.39 & 0.1330 \\
PaddleOCR-VL-1.5~\hfilll~\cite{PaddleOCR-VL-1.5} & specialized & $0.9$\,B & 94.93 & 0.0380 & 96.89 & 91.67 & 94.37 & 0.1300 \\
HunyuanOCR-1.5~\hfilll~\cite{HunyuanOCR-1.5} & specialized & $1$\,B & 94.74 & 0.0390 & 94.50 & 93.67 & 94.71 & 0.1290 \\
PaddleOCR-VL~\hfilll~\cite{PaddleOCR-VL} & specialized & $0.9$\,B & 94.18 & 0.0400 & 95.91 & 90.65 & 93.74 & 0.1350 \\
Qianfan-OCR~\hfilll~\cite{Qianfan-OCR} & specialized & $4$\,B & 93.90 & 0.0400 & 95.08 & 90.53 & 93.31 & 0.1300 \\
\OurMethodV1~\hfilll~\cite{Youtu-Parsing} & specialized & $2.5$\,B & 93.74 & 0.0440 & 93.63 & 92.02 & 95.00 & 0.1160 \\
Ovis2.6-30B-A3B~\hfilll~\cite{Ovis2.5} & general & $30$\,B-A$3$\,B & 93.70 & 0.0350 & 95.17 & 89.44 & 92.40 & 0.1350 \\
Logics-Parsing-v2~\hfilll~\cite{Logics-Parsing} & specialized & $4$\,B & 93.33 & 0.0410 & 95.65 & 88.42 & 91.98 & 0.1370 \\
ABot-OCR~\hfilll~\cite{ABot-OCR} & specialized & $2$\,B & 93.30 & 0.0370 & 94.86 & 88.69 & 91.87 & 0.1370 \\
FireRed-OCR~\hfilll~\cite{FireRed-OCR} & specialized & $2$\,B & 93.26 & 0.0370 & 95.44 & 88.04 & 91.06 & 0.1310 \\
MinerU2.5~\hfilll~\cite{MinerU2.5} & specialized & $1.2$\,B & 93.04 & 0.0450 & 95.77 & 87.88 & 91.47 & 0.1300 \\
Gemini-3-Pro~\hfilll~\cite{Gemini-3} & general & -- & 92.91 & 0.0640 & 95.99 & 89.15 & 92.96 & 0.1650 \\
Gemini-3-Flash~\hfilll~\cite{Gemini-3-Flash} & general & -- & 92.62 & 0.0660 & 95.16 & 89.29 & 93.51 & 0.1720 \\
dots.ocr~\hfilll~\cite{dots.ocr} & specialized & $3$\,B & 90.77 & 0.0480 & 89.95 & 87.18 & 90.58 & 0.1380 \\
OpenDoc-0.1B~\hfilll~\cite{OpenDoc-0.1B} & specialized & $0.1$\,B & 90.67 & 0.0490 & 93.02 & 83.88 & 87.45 & 0.1400 \\
DeepSeek-OCR~2~\hfilll~\cite{DeepSeek-OCR-2} & specialized & $3$\,B & 90.25 & 0.0500 & 91.84 & 83.89 & 87.75 & 0.1440 \\
HunyuanOCR~\hfilll~\cite{HunyuanOCR} & specialized & $1$\,B & 89.95 & 0.0880 & 87.68 & 91.01 & 93.23 & 0.1710 \\
Qwen3-VL-235B~\hfilll~\cite{Qwen3-VL} & general & $235$\,B-A$22$\,B & 89.78 & 0.0630 & 92.55 & 83.07 & 86.75 & 0.1660 \\
Dolphin-v2~\hfilll~\cite{Dolphin} & specialized & $3$\,B & 89.50 & 0.0690 & 91.01 & 84.40 & 87.44 & 0.1500 \\
OCRVerse~\hfilll~\cite{OCRVerse} & specialized & $4$\,B & 88.60 & 0.0630 & 89.61 & 82.44 & 86.27 & 0.1630 \\
MonkeyOCR-pro-3B~\hfilll~\cite{MonkeyOCR} & specialized & $3$\,B & 88.57 & 0.0740 & 88.74 & 84.35 & 88.62 & 0.1890 \\
GPT-5.2~\hfilll~\cite{GPT-5.2} & general & -- & 86.59 & 0.1140 & 88.21 & 82.95 & 87.93 & 0.1930 \\
Dolphin-1.5~\hfilll~\cite{Dolphin} & specialized & $0.3$\,B & 86.52 & 0.0940 & 87.49 & 81.43 & 84.82 & 0.1670 \\
MinerU-Pipeline~\hfilll~\cite{MinerU} & pipeline & -- & 86.47 & 0.0550 & 83.07 & 81.88 & 88.68 & 0.1530 \\
olmOCR~\hfilll~\cite{olmOCR} & specialized & $7$\,B & 85.74 & 0.1390 & 88.10 & 83.00 & 87.17 & 0.2160 \\
Mistral OCR~\hfilll~\cite{Mistral-OCR} & specialized & -- & 85.66 & 0.0970 & 89.91 & 76.78 & 80.93 & 0.1710 \\
Kimi K2.5~\hfilll~\cite{Kimi-K2.5} & general & $1{,}000$\,B-A$32$\,B & 84.53 & 0.1070 & 83.50 & 80.76 & 84.00 & 0.2110 \\
InternVL3.5-241B~\hfilll~\cite{InternVL3.5} & general & $241$\,B-A$28$\,B & 83.76 & 0.1300 & 89.95 & 74.35 & 79.78 & 0.2150 \\
Nanonets-OCR-s~\hfilll~\cite{Nanonets-OCR-s} & specialized & $3$\,B & 83.61 & 0.1080 & 81.46 & 80.18 & 84.51 & 0.2130 \\
POINTS-Reader~\hfilll~\cite{POINTS-Reader} & specialized & $3$\,B & 83.37 & 0.0960 & 85.72 & 73.98 & 77.40 & 0.1980 \\
Marker~\hfilll~\cite{Marker} & pipeline & -- & 78.44 & 0.1570 & 85.24 & 65.77 & 73.24 & 0.2430 \\
\midrule
\rowcolor{youtuBlue!7}\oursmark\OurMethodBF & omni-modal parser & $5$\,B & \best{96.96} & 0.0271 & 96.80 & \second{96.79} & \best{98.20} & \best{0.1104} \\
\bottomrule
\end{tabular}}
\end{table}


==> tables/general.tex <==
\begin{table}[!t]
\centering
\caption{\textbf{On general image benchmarks the model stays inside the range of $2$--$8$B models; on ASR it trails dedicated omni models on the harder English and the Mandarin sets.} Top: general multimodal image benchmarks against $2$--$4$B models (\OurMethod has $5$B parameters). OCRBench is out of $1{,}000$ and enters the six-benchmark mean rescaled by $1/10$. Bold: best; underlined: second best. Middle: additional general VQA benchmarks, all accuracy (\%, higher is better) on the standard splits. Bottom: ASR error rates (\%, lower is better; WER for English, CER for Chinese). Baseline numbers are drawn from publicly reported results.
}
\label{tab:general}
\small
\setlength{\tabcolsep}{5pt}

\begin{tabular}{l cccccc c}
\toprule
\tabhead Model & MMBench & MMStar & MMMU & HallusionBench & AI2D & OCRBench & Avg-6 \\
\midrule
InternVL2.5-4B~\hfilll~\cite{InternVL2.5} & 78.2 & 58.7 & 51.8 & 46.6 & 81.4 & 820 & 66.5 \\
Qwen2.5-VL-3B~\hfilll~\cite{Qwen2.5-VL} & 76.8 & 56.3 & 51.2 & 46.6 & 81.4 & 828 & 65.9 \\
Ovis2-4B~\hfilll~\cite{Ovis} & \underline{81.4} & 61.9 & 49.0 & 53.8 & \best{85.7} & \best{911} & \underline{70.5} \\
InternVL3-2B~\hfilll~\cite{InternVL3} & 78.0 & 61.1 & 48.7 & 41.9 & 78.6 & 831 & 65.2 \\
MiniCPM-V-4.0~\hfilll~\cite{MiniCPM-V} & 79.7 & 62.8 & 51.2 & 50.8 & 82.9 & 894 & 69.5 \\
InternVL3.5-4B~\hfilll~\cite{InternVL3.5} & 80.3 & \underline{65.0} & \best{66.6} & 44.8 & 82.6 & 822 & 70.3 \\
Ovis2.5-2B~\hfilll~\cite{Ovis2.5} & 79.2 & \best{69.8} & \underline{59.8} & \underline{59.2} & \underline{85.5} & 881 & \best{73.6} \\
SAIL-VL2-2B~\hfilll~\cite{SAIL-VL2} & \best{86.8} & 64.1 & 47.7 & 51.7 & 83.0 & \underline{895} & \underline{70.5} \\
\midrule
\rowcolor{youtuBlue!7}\oursmark\OurMethodBF & 81.3 & 58.9 & 50.4 & \best{67.8} & 82.4 & 750 & 69.3 \\
\bottomrule
\end{tabular}
\\[6pt]
\begin{tabular}{l ccccccc}
\toprule
\tabhead Model & POPE & SEED & SciQA & BLINK & MMT-Bench & RealWorldQA & ChartQA \\
\midrule
Qwen2.5-VL-7B~\hfilll~\cite{Qwen2.5-VL}        & 86.48 & \underline{77.15} & 85.13 & 54.66 & 61.05 & 68.63 & -- \\
Qwen2.5-Omni-7B~\hfilll~\cite{Qwen2.5-Omni}    & 86.87 & 76.48 & 85.47 & 54.66 & \best{62.30} & \best{70.98} & -- \\
InternVL2.5-8B~\hfilll~\cite{InternVL2.5}      & \best{90.60} & -- & -- & \underline{54.80} & \best{62.30} & 70.10 & -- \\
LLaVA-OneVision-1.5-8B~\hfilll~\cite{LLaVA-OneVision-1.5} & -- & \best{77.30} & \best{95.00} & -- & -- & 68.10 & \best{86.50} \\
\midrule
\rowcolor{youtuBlue!7}\oursmark\OurMethodBF & \underline{88.18} & 77.11 & \underline{91.87} & \best{62.65} & \underline{61.56} & \underline{70.20} & \underline{83.52} \\
\bottomrule
\end{tabular}
\\[6pt]
\begin{tabular}{l cc >{\columncolor{youtuBlue!7}}c}
\toprule
\tabhead  & Qwen2.5-Omni~\hfilll~\cite{Qwen2.5-Omni} & VITA-Audio~\hfilll~\cite{VITA-Audio} & \oursmark\OurMethodBF \\
\midrule
LibriSpeech test-clean  & 2.37 & \best{2.00} & 2.33 \\
LibriSpeech test-other  & \best{4.21} & 4.60 & 6.12 \\
AISHELL-1          & \best{1.13} & 1.94 & 2.40 \\
WenetSpeech test-meeting & 7.71 & \best{7.12} & 11.44 \\
WenetSpeech test-net    & \best{6.04} & 6.90 & 8.19 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/omniparsingbench.tex <==
\begin{table}[!t]
\centering
\caption{\textbf{Results on OmniParsingBench.} Ovr., Perc., and Cog.\ denote the Overall, Perception, and Cognition scores defined in App.~\ref{subsec:eval-protocol-omniparsing}; all are percentages and higher is better. Bold and underlined entries mark the best and second-best result in each column among the models for which the score is available.}
\label{tab:omniparsing-pc}
\small
\begin{adjustbox}{max width=0.99\textwidth}
\begin{tabular}{lccccccccccccccc}
\toprule
\multirow{2}{*}[-1.0ex]{Model}
& \multicolumn{3}{c}{Natural Image}
& \multicolumn{3}{c}{Graphics}
& \multicolumn{3}{c}{Audio}
& \multicolumn{3}{c}{Natural Video}
& \multicolumn{3}{c}{Text-Rich Video} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
& Ovr. & Perc. & Cog.
& Ovr. & Perc. & Cog.
& Ovr. & Perc. & Cog.
& Ovr. & Perc. & Cog.
& Ovr. & Perc. & Cog. \\
\midrule
Logics-Parsing-Omni
& \underline{67.53} & \underline{43.27} & \textbf{91.79}
& 85.50 & 77.42 & \textbf{93.58}
& 75.58 & 58.23 & \textbf{92.94}
& 67.34 & 44.38 & 90.30
& 65.36 & 36.67 & \underline{94.06} \\
Qwen3-Omni-30B-A3B
& 59.35 & 35.25 & 84.29
& 72.84 & 65.08 & 82.66
& 75.23 & 62.29 & 88.17
& 65.19 & 41.58 & 88.80
& 59.59 & 30.06 & 91.06 \\
Qwen3.5-397B-A17B
& 63.87 & 41.79 & 85.95
& 82.84 & 75.91 & 89.91
& -- & -- & --
& -- & -- & --
& -- & -- & -- \\
Gemini-3-Pro
& \textbf{69.73} & \textbf{48.39} & \underline{91.07}
& \textbf{89.11} & \textbf{86.74} & 91.65
& \underline{76.74} & \textbf{65.74} & 87.90
& \textbf{74.82} & \textbf{58.07} & \underline{91.57}
& \textbf{76.80} & \textbf{60.56} & 93.05 \\
GPT-5.4
& 60.50 & 33.48 & 88.26
& \underline{86.04} & 79.64 & \underline{92.45}
& -- & -- & --
& -- & -- & --
& -- & -- & -- \\
\midrule
\rowcolor{youtuBlue!7}\oursmark\OurMethodBF & 62.84 & 37.52 & 88.15 & 84.68 & \underline{80.31} & 89.23 & \textbf{78.08} & \underline{63.77} & \underline{92.39} & \underline{74.18} & \underline{54.67} & \textbf{93.69} & \underline{75.62} & \underline{56.63} & \textbf{94.60} \\
\bottomrule
\end{tabular}%
\end{adjustbox}
\end{table}


==> tables/pt_stages.tex <==
\begin{table}[!t]
\centering
\small
\caption{Pre-training curriculum.
``fusion layers'' is the number of \OurEncoder layers that receive the group-wise segmentation $\mathbf{c}^{\mathrm{fus}}$ of Subsec.~\ref{subsec:omni-video}.}
\label{tab:pt-stages-full}
\begin{tabular}{lcccc}
\toprule
 & Stage~0 & Stage~1 & Stage~2 & Stage~3 \\
 & perception alignment & omni-modal pre-training & annealing & long-context extension \\
\midrule
trainable          & encoder only & all & all & all \\
\midrule
sequence length    & $4{,}096$ & $8{,}192$--$32{,}768$ & $32{,}768$ & $131{,}072$ \\
tokens / step      & $2^{24}$ & $2^{26}$ & $2^{26}$ & $2^{26}$ \\
tokens (total)     & $320$\,B & $1.28$\,T & $512$\,B & $128$\,B \\
\midrule
max / min LR      & $5\!\cdot\!10^{-4}$ / $5\!\cdot\!10^{-4}$
                   & $10^{-4}$ / $10^{-4}$
                   & $10^{-4}$ / $10^{-5}$
                   & $10^{-5}$ / $10^{-5}$ \\
schedule           & constant & constant & cosine & constant \\
encoder LR decay $\gamma$ & $1.0$ & $1.0$ & $0.9$ & $0.9$ \\
\midrule
fusion layers      & $0$ of $28$ & $4$ of $28$ & $4$ of $28$ & $4$ of $28$ \\
fusion prob.\ $p_{\mathrm{fus}}$ & $1.0$ & $1.0$ & $0.8$ & $0.8$ \\
audio merge $m_a$  & $2$ & $2$ & $2$ & $2$ \\
\midrule
image tokens       & $\le 256$ & $\le 20{,}480$ & $\le 24{,}576$ & $\le 102{,}400$ \\
video frames       & $\le 16$ & $\le 64$ & $\le 64$ & $\le 512$ \\
video tokens       & $\le 2{,}048$ & $\le 20{,}480$ & $\le 24{,}576$ & $\le 102{,}400$ \\
per-frame tokens   & $\le 128$ & $\le 512$ & $\le 1{,}024$ & $\le 1{,}024$ \\
\midrule
tensor parallel    & $1$ & $4$ & $4$ & $8$ \\
recomputation      & none & none & none & decoder + encoder \\
\bottomrule
\end{tabular}
\end{table}


==> tables/token_cost.tex <==
\begin{table}[!t]
\centering
\small
\caption{\textbf{Audio is cheap and video is expensive: a minute of speech costs fewer decoder tokens than four $448\times448$ images.} Token cost per input, derived from Tab.~\ref{tab:arch-config-appx}.
Encoder tokens are charged at the native patch/frame rate; decoder tokens are the merged count that enters the language model.
The video rows include the soundtrack at $1$\,fps.
The per-second rows are rates rather than admissible inputs (the minimum audio chunk is $2$\,s); audio is charged at $13$ tokens per second.}
\label{tab:token-cost}
\begin{tabular}{lrr}
\toprule
Input & Encoder tokens & Decoder tokens \\
\midrule
$448\times448$ image                    & 784     & 196 \\
$8192\times4096$ image, at the token cap & 131{,}072  & 32{,}768 \\
\midrule
$1$\,s of speech                        & 13      & 13 \\
$30$\,s audio chunk                     & 390     & 390 \\
\midrule
$1$\,s of $512\times512$ video           & 1{,}037 & 269 \\
$128$\,s of $512\times512$ video, at the clip cap & 132{,}736  & 34{,}432 \\
\bottomrule
\end{tabular}
\end{table}

